Transferring Rich Feature Hierarchies for Robust Visual Tracking

Convolutional neural network (CNN) models have demonstrated great success in various computer vision tasks including image classification and object detection. However, some equally important tasks such as visual tracking remain relatively unexplored. We believe that a major hurdle that hinders the application of CNN to visual tracking is the lack of properly labeled training data. While existing applications that liberate the power of CNN often need an enormous amount of training data in the order of millions, visual tracking applications typically have only one labeled example in the first frame of each video. We address this research issue here by pre-training a CNN offline and then transferring the rich feature hierarchies learned to online tracking. The CNN is also fine-tuned during online tracking to adapt to the appearance of the tracked target specified in the first video frame. To fit the characteristics of object tracking, we first pre-train the CNN to recognize what is an object, and then propose to generate a probability map instead of producing a simple class label. Using two challenging open benchmarks for performance evaluation, our proposed tracker has demonstrated substantial improvement over other state-of-the-art trackers.

==> intro.tex <==
\section{Introduction}

The last two years have been exciting in the history of computer vision. This excitement has been mainly driven by biologically inspired convolutional neural networks (CNNs) which are trained in a supervised manner through backpropagation of errors. This theme has led to breakthrough performance on several high-level vision tasks such as image classification~\cite{alexnet} and object detection~\cite{rcnn}. However, some important research areas remain unexplored in this surge and one of them is visual tracking. Why is that? We believe the biggest driving force behind CNNs is their ability to learn with large-scale datasets (e.g., millions of images). In the case of visual tracking, however, we typically have only very few examples for training (in fact mostly we only have one single labeled example).  This makes the direct applying of the large-scale CNN approach infeasible. In this paper, we present an approach to overcoming this problem and hence bringing the CNN framework to visual tracking. Our approach demonstrates state-of-the-art performance which outperforms the nearest baseline by more than $10\%$ (see Fig.~\ref{fig:teaser} for some qualitative tracking results).

\begin{figure}[t]
	\center{
	\includegraphics[width=0.32\linewidth]{motocross1_35}
	\includegraphics[width=0.32\linewidth]{motocross1_50}
	\includegraphics[width=0.32\linewidth]{motocross1_75}\\
	\includegraphics[width=0.32\linewidth]{motocross1_105}
	\includegraphics[width=0.32\linewidth]{motocross1_125}
	\includegraphics[width=0.32\linewidth]{motocross1_160}\\
	\vspace{2mm}
	\includegraphics[width=0.32\linewidth]{skiing_6}
	\includegraphics[width=0.32\linewidth]{skiing_15}
	\includegraphics[width=0.32\linewidth]{skiing_28}\\
	\includegraphics[width=0.32\linewidth]{skiing_35}
	\includegraphics[width=0.32\linewidth]{skiing_45}
	\includegraphics[width=0.32\linewidth]{skiing_68}\\
	\vspace{2mm}
	\includegraphics[width=0.6\linewidth]{legend_video}\\

	\caption{Tracking results on \emph{motocross1} and \emph{skiing} sequences.}\label{fig:teaser}
	}
\end{figure}


Although visual tracking can be formulated under different settings, we focus on the \emph{one-pass model-free single object tracking} setting in this paper. That is, we assume that the bounding box of one single object in the first frame is given but no other appearance model is available. Given a single (labeled) instance, the goal is to track the object in an online manner. Therefore, this setting involves adapting the tracker to appearance changes of the object based on the possibly noisy output of the tracker. Another way to formulate this problem would be as a self-taught one-shot learning problem in which the single example comes from the previous frame. Since learning a visual model from a single example is an ill-posed problem, a successful approach would require using some external data to learn an invariant representation of generic object features to exploit. Although there is some recent work~\cite{dlt, wang2012transferring} that shares this spirit, the performance is severely hampered by the lack of sufficient training data and using an improper model. This is where CNN has a role to play. We propose to exploit the scalability of CNN to learn a good set of object features and then transfer the features learned offline for the task of visual tracking.


%In the last two years, we have witnessed great revolution of computer vision: Deep learning, especially \emph{convolutional neural network}~\cite{} (CNN) demonstrates breakthrough performance in high level vision tasks such as image classification~\cite{}, object detection~\cite{}, face recognition~\cite{}. However, the performance is highly relied on huge number of training samples. It is still an open problem to see how CNN works on task with few training samples, such as visual tracking.


%Visual tracking (a.k.a. object tracking) refers to the problem that automatically estimates the states (position, scale, etc.) of objects of interest in a video given their initial states in the first frame. It is a fundamental and crucial problem in computer vision, and has wide applications in video surveillance, robotics planning, human computer interaction, etc. Though numerous methods have been proposed in the past decades, the performance of visual tracking is still far from satisfaction due to the challenges such as occlusion, illumination changes, fast motion, cluttered background  in the video. 
  
% Along this line, xxx~\cite{} proposed to transfer an offline trained SIFT dictionary into online tracking, and showed promising results. Recently, xxx~\cite{} proposed \emph{deep learning tracker} (DLT), which first uses a stacked denoising autoencoder~\cite{} to learn image features offline, and then the encoder part serves as a feature extractor in online tracking. Compared to~\cite{}, the advantage of DLT lies in that the feature extractor is learned from big data, rather than hand-crafted, and it can be further tuned on the fly to better adapt the tracked object in the online process. Though using very simple classifier, DLT showed competitive results with state-of-the-art trackers.

To summarize, we propose a novel structured output CNN that transfers generic object features for online tracking. To prevent overfitting (and drifting at test time), the CNN is pre-trained to distinguish objects from non-objects instead of simply reconstructing the input on large-scale object-level annotation datasets~\cite{imagenet}. During online tracking, the CNN is further tuned to adapt to the specific object being tracked. Furthermore, the output of the CNN is a pixel-wise map to indicate the probability that each pixel in the input image belongs to an object. The key advantages of the pixel-wise output are its induced structure loss and computational scalability. Since the output corresponds to a pixel probability map, first we could model the similarity between bounding boxes better, second we do not need to follow a proposal verification procedure in which hundreds of windows have to be tested at each frame. The pipeline of our tracking algorithm is depicted in Fig.~\ref{fig:pipeline}. We evaluate our proposed algorithm on one open benchmark~\cite{benchmark} and one challenging non-rigid object tracking dataset and show that our method significantly outperforms other state-of-the-art trackers.

%Note that thanks to the  output, we don't need to feed hundreds of proposals to CNN to test, which admits the use of much more powerful model without sacrifice the speed. 


% Next, a multi-scale search scheme on the probability map is designed to find the state of the tracked object. 


